Architecting Optically-Controlled Phase Change Memory

Phase Change Memory (PCM) is an attractive candidate for main memory as it offers non-volatility and zero leakage power, while providing higher cell densities, longer data retention time, and higher capacity scaling compared to DRAM. In PCM, data is stored in the crystalline or amorphous state of the phase change material. The typical electrically-controlled PCM (EPCM), however, suffers from longer write latency and higher write energy compared to DRAM and limited multi-level cell (MLC) capacities. These challenges limit the performance of data-intensive applications running on computing systems with EPCMs. Recently, researchers demonstrated optically-controlled PCM (OPCM) cells, with support for 5 bits/cell in contrast to 2 bits/cell in EPCM. These OPCM cells can be accessed directly with optical signals that are multiplexed in high-bandwidth-density silicon-photonic links. The higher MLC capacity in OPCM and the direct cell access using optical signals enable an increased read/write throughput and lower energy per access than EPCM. However, due to the direct cell access using optical signals, OPCM systems cannot be designed using conventional memory architecture. We need a complete redesign of the memory architecture that is tailored to the properties of OPCM technology. This paper presents the design of a unified network and main memory system called COSMOS that combines OPCM and silicon-photonic links to achieve high memory throughput. COSMOS is composed of a hierarchical multi-banked OPCM array with novel read and write access protocols, and uses an Electrical-Optical-Electrical (E-O-E) control unit to interface with the processor. Our evaluation of a 2.5D-integrated system containing a processor and COSMOS demonstrates 2.14x average speedup compared to an EPCM system. COSMOS consumes 3.8x lower read energy-per-bit and 5.97x lower write energy-per-bit compared to EPCM.

==> Makefile <==
PAPER = main

# for absolute paths: base_dir = $(abspath .)
base_dir = .
build_dir = $(base_dir)/build
src_dir = $(base_dir)

TEX = $(wildcard $(src_dir)/*.tex)
BIB = $(src_dir)/refs.bib
FIGS = $(shell find figures)

LATEX_FLAGS := $(LATEX_FLAGS) \
	--output-directory $(build_dir)

LATEX_ENV := $(LATEX_ENV) \
	TEXINPUTS=$(TEXINPUTS):$(src_dir) \
	BSTINPUTS=$(BSTINPUTS):$(src_dir) \
	BIBINPUTS=$(BIBINPUTS):$(src_dir)

latex = env $(LATEX_ENV) pdflatex $(LATEX_FLAGS)
bibtex = env $(LATEX_ENV) bibtex

vpath %.tex $(src_dir)

.PHONY: all clean

all: $(build_dir)/$(PAPER).pdf

$(build_dir)/$(PAPER).pdf: $(src_dir)/$(PAPER).tex $(TEX) $(BIB) $(FIGS) | $(build_dir)
	$(latex) $<
	$(bibtex) $(build_dir)/$(PAPER)
	$(latex) $<
	$(latex) $<

$(build_dir):
	mkdir $@

clean:
	rm -rf $(build_dir) $(PAPER).pdf

